Interactive Abstract Interpretation: Reanalyzing Whole Programs for Cheap

To put static program analysis at the fingertips of the software developer, we propose a framework for interactive abstract interpretation. While providing sound analysis results, abstract interpretation in general can be quite costly. To achieve quick response times, we incrementalize the analysis infrastructure, including postprocessing, without necessitating any modifications to the analysis specifications themselves. We rely on the local generic fixpoint engine TD, which dynamically tracks dependencies, while exploring the unknowns contributing to answering an initial query. Lazy invalidation is employed for analysis results affected by program change. Dedicated improvements support the incremental analysis of concurrency deficiencies such as data-races. The framework has been implemented for multithreaded C within the static analyzer Goblint, using MagpieBridge to relay findings to IDEs. We evaluate our implementation w.r.t. the yard sticks of response time and consistency: formerly proven invariants should be retained - when they are not affected by the change. The results indicate that with our approach, a reanalysis after small changes only takes a fraction of from-scratch analysis time, while most of the precision is retained. We also provide examples of program development highlighting the usability of the overall approach.

==> content/A-local.tex <==
\section{Restarting in Top-Down Solving}

In this Appendix, we explore some interesting properties of the Top-Down solver.
We show that the restart strategy of \citet{Amato2016} can be applied for the TD solver,
and with such restart, constraint solving is from-scratch consistent for reducible flow graphs.
Our framework is thus from-scratch consistent in the presence of dynamic function calls
in the presense of widening as well as narrowings.

In constraint-based static analysis, the problem is that when widening points are fixed,
inner loops can pick up spurious information about variables manipulated in the outer loop,
and thus apply widenings that the narrowing phase cannot recover from.
\citet{Halbwachs12} showed that restarting the fixpoint iteration for a subset of unknowns
would yield a more precise solution. \citet{Amato2016} showed that such restarting can be achieved
by localizing the application of the widening/narrowing operations, meaning that widening
points are removed when a stable solution is reached for the inner loop.
\citet{Apinis16} integrates localized widenings into the TD solver,
but this is not included in subsequent developments~\cite{DBLP:conf/ppdp/SeidlV18,Seidl2020}.

\begin{figure}
  \centering
  \begin{lstlisting}[xleftmargin=8mm]
    i = 0;
    while (TRUE) {
      i = i + 1;
      j = 0;
      while (j < 10) {
        // Inv: 1 <= i <= 10
        j = j + 1;
      }
      if (i > 9) i = 0;
    }
  \end{lstlisting}
  \caption{Example program \textsf{hybrid} from \citet{Halbwachs12}.}
  \label{f:hybrid}
\end{figure}

Localization alone, however, does not suffice to achieve the same precision as restarting, see example
in \cref{f:hybrid}. Explain the example!

Here, we also incorporate the restarting strategy in the TD solver by restarting whenever
a widening point is first discovered. This computes precise enough information to handle the
assertions in the example.
Together with localization, this achieves the necessary restarting to compute, for reducible flow-graphs,
the equivalent of nested application of fixpoints in the structured denotational approach of, e.g., Cousot and Mine.
This is the intuition for the proof of from-scratch consistency for reducible flow-graphs.

I got somewhat derailed thinking about termination. For SLR, restarting can result in non-termination,
but here we do not switch whenever precision is improved but only when a widening point is first discovered.
This should imply termination because widening points are only removed when inner loop is stable.

Does it also follow that top-down solving without local restart has no chance of being from-scratch consistent?
What of non-reducible flow-graphs?
What of side-effects...

==> content/B-warnings.tex <==
\section{Incremental warning generation}
In \textsc{Goblint}, warnings are generated after the fixed-point iteration has finished.
The reason that warning generation is not done during the solving is that widening may introduce spurious values, that narrowing may later improve upon, leading to fewer warnings.
% E.g.\ the abstract value of an operand for an arithmetic operation may be imprecise after a widening operation has been performed, such that an integer overflow in the operation cannot be excluded. A latter narrowing might yield a more precise result, so that the integer overflow can be excluded.

In this appendix, we describe how the incremental analysis
keeps track of a set of abstract unknowns that are known to be unaffected by the program change. For these, the warning generation does not have to be performed again. \textsc{Goblint} then only needs to communicate newly introduced and removed warnings to user-interfaces (e.g.\ IDEs), making also this part of the workflow incremental.

To this end, we introduce a set $superstable$ that keeps track of unknowns whose abstract values were not modified during the incremental run.
This $superstable$ set is initially created as a copy of the loaded $stable$ set.
The implementation of \lstinline|destabilize| is adapted to  remove unknowns not just from $stable$ but also from $superstable$.
Before the call to \lstinline|solve| in the incremental run, start unknowns of the previous run that are not start unknowns for the current program version, are destabilized.

The disadvantage of this destabilization of obsolete start unknowns is that unknowns that could be reused are removed from stable, thus making a fresh fixed-point iteration for them necessary.


==> content/C-more-background.tex <==

\section{More background}

\subsection{Computation Trees}
The implementation of right-hand sides has to obey certain purity conditions, to be suited for the usage in actual constraint solvers. Being expressible as strategy trees presented as follows is one sufficient condition.

A right-hand side has the form $f: \X \rightarrow (\X \rightarrow \D) \rightarrow \D \times (\X \rightarrow \D)$.
We demand that right-hand sides are pure second-order functionals in the sense of \cite{DBLP:phd/dnb/Karbyshev13}, and thus are expressible as \textit{strategy trees} of the following form \cite{DBLP:conf/ppdp/SeidlV18}:

\[
    \mathcal{T} = Ans\;\D\;|\;QGet\;(X , \D \rightarrow \mathcal{T})\;|\;QSet\;(X , \D, \mathcal{T})
\]

The semantic of computation trees can then be defined relative to a state $S = (X \rightarrow \D) \times 2^{X} \times (\X \rightarrow \D)$ and functions $get: X \rightarrow  S \rightarrow S \times \D$ and $set: \X \rightarrow \D \rightarrow S \rightarrow S \times \bullet $, that allow to query the value of an unknown and to add a contribution
to an unknown, respectively.

The tree $Ans\;d$ immediately returns the answer $d$. The tree $QGet\;(x , f)$ retrieves the value of $x$, and passes the received value to the continuation function $f$.
The tree $QSet\;(x, d, t)$ adds the value
$d$ to the side effect function in the state and passes the resulting state to the continuation defined by $t$.

Formally, the semantics of strategy trees
can be defined using state monads.

The state monad $M_S(A) = S \rightarrow S \times A$ of a type $S$ of states and values of type $A$ is defined by the functions
$\return : A \rightarrow M_S(A)$ and $\bind : M_S(A) \rightarrow (A \rightarrow M_S(B)) \rightarrow M_S(B)$.
\[
\begin{array}{lll}
\return\;a\;s & = &  (s, a) \\
\bind\;m\;f\;s & = &
 \textbf{let}\;(s', a) = m\;s\;\textbf{in}\\
& & f\;a\;s'
\end{array}
\]

The semantics of strategy trees of type $\Tt$ is defined as the transformation on a state monad, relative to the functions $get$ and $set$. Thus, the semantics are defined via a function $\sem{t}:(X \rightarrow  \M_S{\D}) \rightarrow (X \rightarrow \D \rightarrow \M_S(\bullet)) \rightarrow \M_S(D)$.

\[
\begin{array}{lll}
    \sem{Ans\;d}~get~set~s & = & (s, d) \\
    \sem{QGet\;(x, f)}~get~set~s & =
    & \Let~(s', d) = get~x~s~\In \\
    & & f ~ d ~ s' \\
    \sem{QSet\;(x,d,t)}~get~set~s & =
    & \Let~(s', ()) = set~x~d~\In \\
    & & \sem{t}~get~set~s' \\
\end{array}
\]

The functions $get$ and $set$ used here are defined as follows:

\[
\begin{array}{lll}
get~x~(\sigma, X, \rho) & = & ((\sigma, X, \rho), \sigma~x) \\
set~x~d~(\sigma, X, \rho) & =
& \Let~\rho' = \rho\oplus \{ x \mapsto  \rho~x \sqcup d \}~\In \\
& & ((\sigma, X, \rho'), ())
\end{array}
\]

$get$ retrieves the value of $x$ in $\sigma$, and propagates the state unchanged. $set$ modifies the mapping $\rho~ x$ by joining $d$ with the old value of the mapping.

As noted in Proposition 1 of \cite{Seidl2020}, the evaluation of right-hand sides without side-effects is not sensitive in variables that are never queried by the corresponding strategy tree.
For a setting with side effects, i.e. $QSet$ nodes in the strategy tree, the following adapted proposition holds:

\begin{proposition}
For a mapping $\sigma : \X \rightarrow \D$ and $s=(\sigma, \emptyset, \{ \})$, assume that $\sem{t}~get ~set~(s_1, d)$, with $s_1=(\sigma_1, X, \rho)$. The following holds:
\begin{enumerate}
    \item $\sigma = \sigma_1$
    \item Assume that $\sigma': \X \rightarrow \D$ is another mapping with $\sigma'|_X =\sigma|_X $. Let $s' = (\sigma', \emptyset,\{\})$, and let $\sem{t}~get~set~s'= ((\sigma', X', \rho'), d')$. Then $X = X'$, $d =d'$ and $\rho = \rho'$.
\end{enumerate}
\end{proposition}


\subsection{Top-down solver for side-effecting constraint systems}
We base our work on $TD_{side}$, the version the top-down solver that supports side-effecting constraint systems from \cite{DBLP:conf/ppdp/SeidlV18}.
The code can be found in \cref{lst:td_side} in an OCaml like notation.
\begin{lstlisting}[language={[Objective]Caml}, caption={Code of $TD_{side}$, verbatim from \cite{DBLP:conf/ppdp/SeidlV18}}, basicstyle={\footnotesize}, fontadjust=true, basewidth=0.48em, label={lst:td_side}]
(* state / mutable data structures: *)
val |$\sigma\:\,$|     : (|$\X$|, |$\D$|) Map.t
val infl   : (|$\X$|, |$\X$| Set.t) Map.t
val called : |$\X$| Set.t
val stable : |$\X$| Set.t
val point  : |$\X$| Set.t
(* functions on them: *)
val get : 'a -> ('a,'b) Map.t -> 'b
val set : 'a -> 'b -> ('a,'b) Map.t -> unit
val |$\in\:\,$|  : 'a -> 'a Set.t -> bool
val add : 'a -> 'a Set.t -> unit
val rem : 'a -> 'a Set.t -> unit

let destabilize x =
  let w = get x infl in
  set x (Set.create ()) infl;
  iter (fun y ->
    rem y stable;
    if y |$\not\in$| called then
      destabilize y
    ) w

let eval x y =
  if y |$\in$| (called |$\bm{\cup}$| |\textbf{leaf}|) then
    add y point
  else
    solve |$\widen$| y;
  add x (get y infl);
  get y |$\sigma$|

let side x d =
  let tmp = (get x |$\sigma$|) |$\widen$| d in
  if get x |$\sigma$| |$\neq$| tmp then (
    set x tmp |$\sigma$|;
    add x stable;
    destabilize x
  )

let solve p x =
  if x |$\not\in$| (stable |$\cup$| called) then (
    add x stable;
    add x called;
    let tmp = (|$f\s_x$| (eval x) |\textbf{side}|)|$_1$| in
    rem x called;
    let tmp =
      if x |$\in$| point then p (get x |$\sigma$|) tmp
      else tmp
    in
    if x |$\not\in$| stable then solve |$\widen$| x
    else if get x |$\sigma$| = tmp then
      if p = |$\widen$| && x |$\in$| point then (
        rem x stable;
        solve |$\narrow$| x
      ) else ()
    else (
      set x tmp |$\sigma$|;
      destabilize x;
      solve p x
    )
  )
\end{lstlisting}

% %
The function \lstinline{solve} is the core function of $TD_{side}$, that is queried with an initial unknown of interest $x$, evaluates the right-hand side of the unknown and recursively of those unknowns on which it depends, so that a valid improved partial post-solution\todo{define this} is stored in $\sigma$, with $x \in \lstinline |stable|$.

The \lstinline|called| set keeps track of unknowns for which \lstinline|solve| is currently called. To avoid infinite recursion for unknown that cyclically depend on themselves, \lstinline|solve| immediately returns in case it is queried for an unknown in \lstinline|called|.

The \lstinline|stable| set is used to track for which variables the evaluation of the right-hand side under the current $\sigma$ would not yield a different result. % Elaborate on what "evaluation of the right-hand side means here,

When \lstinline|solve| is queried for an unknown $x$, it is "optimistically" added to the \lstinline|stable| set before the right-hand side is evaluated.
This is done so that, in case a (value-changing) side effect on to an unknown $y$ that influences $x$ occurs during the evaluation of the right-hand side for $x$, $x$ is removed from the stable set.
So, after the evaluation of the right-hand side, it can be determined by checking $x \not\in \lstinline|stable|$ whether such a side effect to an influencing unknown occurred.

If this is the case, \lstinline|solve| needs to be recursively called again for $x$. When the recursive call returns, we know that $x \in \lstinline|stable|$.

The right-hand side is evaluated, and the resulting value is stored in $tmp$. In case the unknown was detected to be a widening point,
the operator $p \in \{\widen, \narrow\}$ is performed on the old value of the unknown and $tmp$.

If $x \in \lstinline|stable|$ directly after the evaluation of the right-hand side, it is checked whether the computed value $tmp$ is the
same as the value stored in $\sigma$. If this is the case, and $x$ is a widening point and the current phase is $\widen$, then a narrowing iteration is started for $x$.

Otherwise, i.e. if the value of $tmp$ is not the same as the one in $\sigma$, the mapping in $\sigma$ is updated, $x$ is destabilized, i.e. the unknowns that are influenced by $x$ are recursively removed from $stable$, and \lstinline|solve| is called again for $x$.

The function \lstinline|eval x y| yields a value for the unknown $y$.
In case $y$ is not already called (or doesn't have a right-hand side, i.e. $y \in leaf$ ), it triggers the evaluation of the right-hand side by calling \lstinline|solve| on it.
\lstinline|eval| is meant to be passed as a partially applied function \lstinline|eval x| to the function $f\s_x$ that realizes the right-hand side of $x$.
To record this dependency, $x$ is added to the set of unknowns influenced by $y$.
Finally, the value of $y$ in $\sigma$ is returned.

The function \lstinline|destabilize| takes an unknown $x$ and transitively removes all unknowns that are influenced by it from $stable$ and resets the $infl$ resets of all visited unknowns to the empty set.

The function \lstinline|side| takes an unknown $x$ and a contribution $d$. It performs a widening with the old value of $x$ and $d$, and updates the value in $\sigma$ correspondingly.
In case the value changed, the unknowns (transitively) depending on $x$ are removed from \lstinline|stable|.


==> content/D-IDE-integration.tex <==
\section{IDE-Integration}
\textsc{Goblint} has been chiefly a command-line tool. It also has a web frontend based on \textsc{jsoo-react}, which can visualize the results better than a command-line interface. However, a separate web frontend is not as convenient for the developers as IDE-integrated tools, making it challenging to reach widespread use. Therefore a solution for simple IDE integration was sought.

The \textsc{MagpieBridge} framework \cite{luo_et_al:LIPIcs:2019:10813} aims to provide a generic communication layer between static analysis tools and various Integrated Development Environments.
With \textsc{MagpieBridge} only the binding has to be implemented for a static analysis tool to support a range of IDEs.
%Is this true? - It is written so in their paper, but none of us in Tartu have tried it out on anything other than VSCode. Or is this question about this "only a binding" part? If so, I am not too sure how a binding in CS is defined exactly.
The binding with \textsc{MagpieBridge} implemented for Goblint is GobPie. GobPie communicates with Goblint via Unix socket using JSON-based RPC protocol. GobPie then converts and forwards the results from the \textsc{Goblint} server to \textsc{Magpie} Server, which displays the result into IDEs, therefore bringing sound static program analysis closer to being used by developers day-to-day. On \cref{f:gobpie} a nullpointer dereference warning by Goblint is displayed in the VSCode IDE.

\begin{figure}[t]
    \includegraphics[width=0.45\textwidth]{content/gobpie_IDE.png}
    \caption{Gobpie extension showing nullpointer dereference warning in VSCode IDE}
    \label{f:gobpie}
\end{figure}


==> content/fail.tex <==
Recall that in C11 (as well as in \textsc{Posix} threads), locking of mutexes may fail and is only guaranteed to have succeeded if
the value 0 is returned. 
%
For the analysis of possibly failing locks,
a \emph{lockset} analysis is presented 
in \cite{VojdaniVene09}. 
Besides information on the local state,
this analysis keeps track of the set of definitely acquired mutexes, 
while keeping program states apart when the set of mutexes differ.
%
Thereby, a call $s$ of the form
{\small\begin{lstlisting}
   b = lock(&A);
\end{lstlisting}}
\noindent
for some mutex $A$ 
is modeled abstractly 
as the non-deterministic choice between the two abstract transformers $\sem{s}_+^\sharp$ and $\sem{s}_-^\sharp$ 
describing successful and failing executions of the statement $s$, respectively. 

% 
Assume that 
%the \emph{lockset} analysis tracks abstract 
local states are of the form $(\sigma,S)$ where $\sigma$ is an abstract variable assignment
and $S$ is a set of (addresses of) mutexes which have successfully been acquired. 
Then 
\[
\begin{array}{lll}
\sem{s}^\sharp_+\,(\sigma,S)	&=& (\sigma\oplus\{b\mapsto 0\},S\cup\{\&A\})	\\
\sem{s}^\sharp_-\,(\sigma,S)	&=& (\sigma\oplus\{b\mapsto \neg 0\},S)	\\
\end{array}
\]
where $\neg 0$ denotes the set of all \lstinline|int| values besides 0.
%
For an illustration of \emph{path-splitting},
consider the code snippet
{\small\begin{lstlisting}
   int b;
   b = lock(&A);
   if (!b) {
     g = 42;
     unlock(&A);
   }
\end{lstlisting}}
\noindent
where $g$ is some shared variable.
%
Let $u_1,u_2$ denote the program points before the \lstinline|if| and the access to $g$, respectively.
%
For these program points, \emph{lockset} analysis without \emph{path-splitting} infers 
abstract states $(\sigma_1,S_1),(\sigma_2,S_2)$, respectively, where
\[
\sigma_1\,b=\top\quad\text{and}\quad \&A\not\in S_1
\]
%
Accordingly, also $\&A\not\in S_2$ -- implying that 
protection of $g$ by $A$ cannot be inferred.

Introducing \emph{path-splitting} on sets of acquired mutexes, however, keeps the two possible outcomes of
the lock operation apart. 
Assume that some abstract state $(\sigma,S)$ arrives at the locking statement for \lstinline|\&A|.
%
Then program point $u_1$ is reached by the two abstract states 
\[
(\sigma\oplus\{b\mapsto 0\},S\cup\{\&A\}),\,
(\sigma\oplus\{b\mapsto \neg 0\},S)
\]
From these, only the first abstract state arrives at the access of global $g$ at node $u_2$.
Accordingly, protection of the given access to $g$ by $A$ is verified.
\qed


==> content/solver.tex <==
\section{Background}\label{s:background}


\begin{figure}

\caption{Overview over the base analyzer}\label{f:base}
\end{figure}

\begin{figure}

\caption{Overview over the interactive analyzer}\label{f:interactive}
\end{figure}

The workflow of a static analyzer such as \textsc{Goblint} (see \cref{f:base}) is organized like a pipeline.
It takes as input the whole program,
transforms it into some internal representation, e.g., a set of control-flow graphs.
Together with the specification of certain analyses (and, perhaps, further options guiding the
analysis process), the fixpoint engine then computes the analysis results, i.e., the
invariants which are valid when reaching program point, the values of globals, warnings concerning
to violations of assertions, etc. which are either persistently stored or displayed in appropriate viewers.
%
In order to allow for an interactive static reanalysis of the code base,
we suggest to close the loop within an IDE which both allows for editing the code and rendering the analysis results.
Moreover, feedback loops are introduced along the analysis pipeline in order to minimize the effort of the
reanalysis.

\todo{More on the general reanalysis infrastructure!}

Subsequently, we concentrate our exposition onto our techniques for restricting reanalysis to the bare minimum.
%
% unknowns introduced for the pieces of information to compute invariants for, e.g.,
% program points (perhaps enhanced with calling-contexts) or
% global variables or
% (classes of) dynamically allocated data-elements
%
% Lattice elements for representing invariant properties, e.g., intervals of values for local variables
%
% semantic dependence between of an unknown $u$ realized by means of a right-hand side function $f_u$ of functionality
% $f_u: ...
%
% The analysis result $\sigma$, $\infl$, $\infl\_\side$
%
% Example
%


==> defs.tex <==
%Copied from https://tex.stackexchange.com/questions/128797/a-renewcommand-that-does-not-care-if-a-command-is-already-defined
\makeatletter
\newcommand*{\declarecommand}{%
  \@star@or@long\declare@command
}
\newcommand*{\declare@command}[1]{%
  \provide@command{#1}{}%
  % \let#1\@empty % would be more efficient, but without error checking
  \renew@command{#1}%
}
\makeatother


\makeatletter

\newcount\comment@nesting

\newenvironment{comment}{%
    \begingroup
    \global\comment@nesting=0
    \def\do##1{\catcode`##1=12\relax}%
    \dospecials
    \catcode`\^^M=\active
    \comment@processline
}{%
    \endgroup
}

\begingroup
\escapechar=-1
\xdef\comment@begincomment{\string\\begin\string\{comment\string\}}
\xdef\comment@endcomment{\string\\end\string\{comment\string\}}
\endgroup

\begingroup
\catcode`\^^M=\active
\def\@temp{\endgroup\def\comment@processline##1^^M}%
\@temp{%
    \def\comment@curline{#1}%
    \let\@next=\comment@processline
    \ifx\comment@curline\comment@endcomment
        \ifnum\comment@nesting=0
            \def\@next{\end{comment}}%
        \else
            \global\advance\comment@nesting by -1
        \fi
    \else
        \ifx\comment@curline\comment@begincomment
            \global\advance\comment@nesting by 1
        \fi
    \fi
    \@next
}

\makeatother

\newcommand{\angl}[1]{\langle #1 \rangle}
\newcommand{\D}{\mathcal{D}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Tt}{\mathcal{T}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\bind}{\textrm{{bind}}}
\newcommand{\return}{\textrm{return}}
\newcommand{\sem}[1]{\llbracket #1 \rrbracket}
\newcommand{\Let}{\textbf{let}}
\newcommand{\In}{\textbf{in}}

\DeclareMathOperator{\s} {^{\#}}
\DeclareMathOperator{\widen} {\nabla}
\DeclareMathOperator{\narrow}{\Delta}

